Privacy-preserving Optics for Enhancing Protection in Face De-identification

The modern surge in camera usage alongside widespread computer vision technology applications poses significant privacy and security concerns. Current artificial intelligence (AI) technologies aid in recognizing relevant events and assisting in daily tasks in homes, offices, hospitals, etc. The need to access or process personal information for these purposes raises privacy concerns. While software-level solutions like face de-identification provide a good privacy/utility trade-off, they present vulnerabilities to sniffing attacks. In this paper, we propose a hardware-level face de-identification method to solve this vulnerability. Specifically, our approach first learns an optical encoder along with a regression model to obtain a face heatmap while hiding the face identity from the source image. We also propose an anonymization framework that generates a new face using the privacy-preserving image, face heatmap, and a reference face image from a public dataset as input. We validate our approach with extensive simulations and hardware experiments.

==> sections/trash.tex <==
\noindent \textit{Experiment I: Face Recognition}
\JL{To assess the robustness of our proposed approach in safeguarding facial anonymity, we conducted a series of experiments focused on face recognition tasks. Specifically, we employed the cutting-edge \textit{AdaFace} neural network architecture as presented by Kim et al. \cite{kim2022adaface}, utilizing LFW \cite{huang2008labeled}, CFP-FP \cite{sengupta2016frontal}, CPLFW \cite{zheng2018cross}, AgeDB \cite{moschoglou2017agedb}, and CALFW \cite{zheng2017cross} datasets. These experiments encompass the following four key scenarios: \\
\begin{enumerate}
\item \textbf{No-Privacy Model:} In this experiment, we utilized the pre-trained AdaFace model to assess the performance on original, unaltered facial images.
\item \textbf{Pretrained Model:} Building upon the previous experiment, we employed the same pre-trained AdaFace model to evaluate its performance on the privacy-enhanced versions of each dataset.
\item \textbf{Trained Model:} To gauge the effectiveness of training AdaFace from scratch on privacy-preserving facial data, we conducted experiments using the private version of the MS1MV2 dataset \cite{deng2019arcface}.
\item \textbf{Fine-Tuned Model:} In this experiment, we fine-tuned the pre-trained AdaFace model using the private version of the MS1MV2 dataset, assessing the model's adaptability to privacy-preserving facial recognition.
\end{enumerate}}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figs/Results/Face_recognition.png}
    \caption{Face recognition performance on images acquired with our optimized lens, compared to different state-of-the-art datasets.}
    \label{fig:face_rec}
\end{figure*}

% ________________________________________________________
The low-resolution camera seems to be a simple and very easy-to-implement alternative to protect people's privacy, but if a scenario where an attacker captures a low-resolution image or our privacy images, they can apply some state-of-the-art algorithms to try to recover the original image. To avoid this scenario, we use the diffusion model (DDRM) proposed by Kawar et al. \cite{kawar2022denoising}, which is trained to recover images in different scenarios, such as superresolution, inpainting, colourization and deblurring over Celeba-HQ and other datasets. We use the pre-trained model over Celeba-HQ dataset to try to recover the privacy images from low resolution and our optimized camera. As shown in Fig. \ref{fig:diff_rstl}, DDRM can recover the original image from a low-resolution private version with high accuracy. On the other hand, when we try to recover low-resolution images, the diffusion model achieves a high performance and can recover the original image with high accuracy; on the contrary, when recovering the private image with our camera, the diffusion model fails. This recovery was obtained by setting the model in Gaussian deblurring mode and assuming that the input images have a standard deviation of 0.17 (this value was obtained by averaging the standard deviations of 1000 private images). Therefore, our designed camera is more robust to this real scenario. 

% --------------------------------------------------------

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{2}{c}{Method}                                                   & Ours & Flow & Land-Flow             & Low Resolution 16 & Low Resolution 32 \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Identity Distance $\uparrow$}} & VGGFace & 1.159     &      & \multicolumn{1}{c|}{} & 1.141             &                   \\
\multicolumn{1}{c|}{}                                              & Casia   & 0.991     &      & \multicolumn{1}{c|}{} & 1.021             &                   \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Bounding box}}                 & MtCNN   & 4.292     &      & \multicolumn{1}{c|}{} & 4.126             &                   \\
\multicolumn{1}{c|}{}                                              & Dlib    & 3.887     &      & \multicolumn{1}{c|}{} & 4.077             &                   \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Landmark}}                     & MtCNN   & 3.196     &      & \multicolumn{1}{c|}{} & 3.094             &                   \\
\multicolumn{1}{c|}{}                                              & Dlib    & 2.160     &      & \multicolumn{1}{c|}{} & 1.995             &                   \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:ablations}
\end{table}

